Finding Convincing Views to Endorse a Claim

Recent studies investigated the challenge of assessing the strength of a given claim extracted from a dataset, particularly the claim's potential of being misleading and cherry-picked. We focus on claims that compare answers to an aggregate query posed on a view that selects tuples. The strength of a claim amounts to the question of how likely it is that the view is carefully chosen to support the claim, whereas less careful choices would lead to contradictory claims. We embark on the study of the reverse task that offers a complementary angle in the critical assessment of data-based claims: given a claim, find useful supporting views. The goal of this task is twofold. On the one hand, we aim to assist users in finding significant evidence of phenomena of interest. On the other hand, we wish to provide them with machinery to criticize or counter given claims by extracting evidence of opposing statements. To be effective, the supporting sub-population should be significant and defined by a ``natural'' view. We discuss several measures of naturalness and propose ways of extracting the best views under each measure (and combinations thereof). The main challenge is the computational cost, as na\"ive search is infeasible. We devise anytime algorithms that deploy two main steps: (1) a preliminary construction of a ranked list of attribute combinations that are assessed using fast-to-compute features, and (2) an efficient search for the actual views based on each attribute combination. We present a thorough experimental study that shows the effectiveness of our algorithms in terms of quality and execution cost. We also present a user study to assess the usefulness of the naturalness measures.

==> 011-Motivating-example.tex <==
\brit{Shunit please change to a table instead of a figure and remove some tuples to save space. also move it to section 2 since it is not discussed in the introduction}
\benny{In my understanding, "table" refers to information that we want to present in a tabular form (e.g., experimental results, comparisons, etc.). But here, the table \textbf{is} the object that we depict, so "Figure" is a better label for what we have here.}

\begin{figure*}[ht]
    \centering \small
    \begin{tabular}{cclcllcc}
        \hline
        \rowcolor{lightgray}ID & Sex & OccupationGroup & Age (binned) & EducationLevel & MaritalStatus & QuarterOfBirth & TotalIncome (K)\\
        \hline
        1 & F & CS\&Math & 30-35 & Bachelor's degree & Never Married & 1 & 72 \\
        2 & F & CS\&Math & 40-45 & Master's degree & Divorced & 3 & 95 \\
        3 & F & Education & 40-45 & Master's degree & Married & 2 & 43 \\
        4 & F & Sales & 40-45 & High School Diploma & Married & 1 & 35 \\
        5 & F & Sales & 30-35 & Bachelor's degree & Never Married & 4 & 100 \\
        6 & M & CS\&Math & 30-35 & Bachelor's degree & Never Married & 4 & 80 \\
        7 & M & CS\&Math & 40-45 & Master's degree & Married & 3 & 90 \\
        8 & M & Education & 40-45 & Master's degree & Married & 2 & 62 \\
        9 & M & Sales & 40-45 & Bachelor's degree & Divorced & 1 & 70 \\
        10 & M & Sales & 40-45 & High School Diploma & Never Married & 3 & 65 \\
        \bottomrule
    \end{tabular}
    \caption{Sample of the ACS dataset~\cite{folktables2021}.}
    \label{tab:DB_example}
\end{figure*}

% \brit{end the example without explaining why the second is more natural, the second part only after talking about naturalness measures}


\begin{example}\label{ex:motivating1}\em
The Stack Overflow developers survey~\cite{so_survey} contains information about workers in the Hi-Tech industry, their background, demographics, and yearly salary. Alex, a social scientist, aims to claim that on average, people with a Master's degree earn more than people with a bachelor's degree. 
However, this claim is false in the dataset: the average income for people with a Master's degree is \$156K, as opposed to \$183K for Bachelor's degree. Alex then seeks subpopulations that support the claim. She discovers that among individuals who want to use Emacs and do not know the size of their organization, those with a Master's degree have a higher average salary than those with a bachelor's degree. However, this definition of subpopulation seems artificial and arbitrary and thus is not convincing.  She also discovers that among individuals living in Germany who have little coding experience, the average income for Master's degree graduates is higher than the average income for Bachelor's degree graduates. Intuitively, this claim seems to Alex as a more appropriate and natural subpopulation supporting her claim. \qed
\end{example}


% \begin{example}\label{ex:motivating1}
% Consider the Stack Overflow survey from 2022~\cite{so_survey}. This dataset contains information about workers in the Hi-Tech industry, their background, demographics, and yearly salary. Consider a claim stating that on average, people with a Master's degree earn more than people with a bachelor's degree. 
% % However, oftentimes the claim is not supported by the data (namely, the average salary of people with a Master's degree is lower than that of people with a bachelor's degree). 
% This statement does not hold for over the entire dataset. In particular, the average income for people with a Master's degree is 156K, as opposed to 183K for Bachelor's degree holders.
% However, there are subsets of the data for which the claim holds. 
% For instance, among individuals who want to use Emacs\footnote{\url{https://en.wikipedia.org/wiki/Emacs}} and do not know the size of their organization, those with a Master's degree have a higher average salary than those with a bachelor's degree. A more \emph{natural} subset validating the claim comprises individuals living in Germany who have little coding experience (under 10 years).
% In this subpopulation, the average income for Master's degree graduates is 126K, while the average income for Bachelor's degree graduates is 104K. 
% Intuitively, this subpopulation appears to be a more appropriate choice because it is \emph{larger} and it is defined by attributes that are more \emph{closely related to the target attribute} salary. For comparison, in the first subpopulation, there are only 20 people, and the average salary for Master's graduates is 71K vs. 70K for bachelor's, which is not a statistically significant difference.
% \end{example}

%\begin{example}\label{ex:motivating2}
%As another example, consider the American Community Survey (ACS)~\cite{folktables2021}\footnote{from 2018, from the top populated 7 states.}. A sample database based on averages from this dataset is shown in \cref{tab:DB_example}.

% Also consider the statement ``Women have a higher income than men''. As found in previous research work \cite{weinberg2004evidence}, the statement is counter-intuitive as there is a gender pay gap if favor of men. In particular, the statement does not hold when considering the full dataset: the total income for women (average=$33,245$, median=$19,300$) is lower than men's (average=$54,493$, median=$32,400$). 
% But the statement does hold on various subsets of the data, some more convincing (or {\em natural}) than others. 
% For example, we could create the following refined statements, which are supported by this dataset: 
% \begin{enumerate}
%     \item ``Among African-Americans of age $19$-$28$, women have a higher average income.''
%     \item ``Among people from California serving in the military, women have a higher average income.''
%     \item \ag{An unnatural statement}
% \end{enumerate}
% For Item (1) the income of males is \ag{X} and the income of females \ag{Y}, and for Item (2) the income of males is \ag{Y} and the income of females \ag{W}.
% While Items (1) and (2) are more natural, Item (3) is more artificial-sounding and less convincing. 
% Our solution is able to discover statements like (1) and (2) when given a dataset and a claim to prove. 
% \ag{Follow the same logic for this example:}
% Another example statement is "People with Bachelor's degree have a higher total income than Master's degree holders". 
% Also consider the hypothesis that, on average, people with a Master's degree earn more than people with a bachelor's degree. However, oftentimes the claim is not supported by the data (namely, the average salary of people with a Master's degree is lower than that of people with a bachelor's degree). 
% This statement does not hold for the full dataset. In particular, people with a Master's degree average total income is 85K, as opposed to 66K for Bachelor's degree holders \ag{This does not match the results specified in \cref{ex:running_example}. Which is true?}. \shunit{These are the numbers from the real ACS dataset. In \cref{ex:running_example} the numbers are based on the example dataset in \cref{tab:DB_example}. In stack overflow, which is maybe a more suitable dataset for this claim, it's 183K for bachelor's vs. 155K for master's.}
% However, there are subsets of the data for which the hypothesis holds. 
% For instance, it might be true that among individuals with blue eyes and red hair, those with a Master's degree have a higher average salary than those with a bachelor's degree. A more \emph{natural} subset validating the claim comprises individuals in high-tech industries with little coding experience  \ag{Shunit, can you verify?}. \shunit{I think you mixed up Stack Overflow with ACS. The details about coding experience are from SO.} 
% In this subpopulation, the average income for Master's degree graduates is \ag{X}, while the average income for Bachelor's degree graduates is \ag{Y}. 
% Furthermore, this subpopulation appears to be a more appropriate choice because it is \emph{large} (its size is \ag{W}) and it is defined by attributes that are more \emph{closely related to the target attribute}, namely salary.
% Indeed, our algorithms are able to detect the latter view as the most convincing example of a view for which the hypothesis holds, when given specific measures of naturalness. 
% In general, there are $1,073,444$ predicates where the statement holds, composed of up to 2 features. For $639,758$ of them, the number of people in each group is larger than 30.


%\end{example}


==> full_mean_q.tex <==
\begin{figure}[htbp]
\centering
\begin{minipage}[b]{1.0\linewidth}
\begin{tcolorbox}[colback=white]
\vspace{-2mm}
\begin{center}
\small
\begin{tabular}{l}
\textsf{blue{SELECT}} $A_1, ..., A_\ell$\\
\textsf{blue{AVG}(CASE WHEN} $Agb=g_1$ \textsf{THEN} $\Aagg$ \textsf{END) \textcolor{blue}{as} mean1,}\\
\textsf{COUNT(CASE WHEN} $\Agb=g_1$ \textsf{THEN} $\Aagg$ \textsf{END) as count1,}\\
\textsf{STDDEV (CASE WHEN} $\Agb=g_1$ \textsf{THEN} $\Aagg$ \textsf{END) as s1,}\\
\textsf{AVG(CASE WHEN} $\Agb=g_2$ \textsf{THEN} $\Aagg$ \textsf{END) as mean2,}\\
\textsf{COUNT(CASE WHEN} $\Agb=g_2$ \textsf{THEN} $\Aagg$ \textsf{END) as count2,}\\
\textsf{STDDEV (CASE WHEN} $\Agb=g_2$ \textsf{THEN} $\Aagg$ \textsf{END) as s2}\\
\textsf{FROM $D$}\\
\textsf{GROUP BY} $A_1, ..., A_\ell$\\
\textsf{HAVING AVG(CASE WHEN} $\Agb=g_1$ \textsf{THEN} $\Aagg$ \textsf{END)<}\\
\textsf{\,\,\,\,\,\,\,\,\,\,\,\,\,\,\,\,\,\,\,\,\,\,\,AVG(CASE WHEN} $\Agb=g_2$ \textsf{THEN} $\Aagg$ \textsf{END)}\\
\textsf{\,\,\,\,\,\,\,\,\,\,\,AND COUNT(CASE WHEN} $\Agb=v_1$ \textsf{THEN} $\Aagg$ \textsf{END>}$M$\\
\textsf{\,\,\,\,\,\,\,\,\,\,\,AND COUNT(CASE WHEN} $\Agb=g_2$ \textsf{THEN} $\Aagg$ \textsf{END)>}$M$;

\end{tabular}
\end{center}
\vspace{-2mm}
\end{tcolorbox}
\end{minipage}%%
\vspace{-4mm}
\caption{Mean aggregation query for a given attribute combination $A_1,\ldots, A_\ell$.}
\label{fig:full_mean_gb_query}
\end{figure}





==> full_median_q.tex <==
\begin{figure}[htbp]
\centering
\begin{minipage}[b]{1.0\linewidth}
\begin{tcolorbox}[colback=white]
\vspace{-2mm}
\begin{center}
\small
\begin{tabular}{l}
\textsf{WITH discretized AS (SELECT} $A_1, ..., A_n, A_p, T$ \textsf{FROM} $D$\textsf{),}\\
\textsf{filtered AS (}\\
\textsf{SELECT} $A_1, ..., A_n$\textsf{,}\\
\textsf{\,\,\,\,PERCENTILE\_CONT(0.5) WITHIN GROUP (}\\
\textsf{\,\,\,\,\,\,\,\,ORDER BY CASE WHEN} $A_p=v_1$ \textsf{OR} $A_p=v_2$ \textsf{THEN} $T$ \textsf{END)}\\ 
\textsf{\,\,\,\,\,\,\,\,AS total\_median,} \\
\textsf{\,\,\,\,PERCENTILE\_CONT(0.5) WITHIN GROUP (}\\
\textsf{\,\,\,\,\,\,\,\,ORDER BY CASE WHEN} $A_p=v_1$ \textsf{THEN} $T$ \textsf{END)}\\
\textsf{\,\,\,\,\,\,\,\,AS median1,}\\
\textsf{\,\,\,\,COUNT(CASE WHEN} $A_p=v_1$ \textsf{THEN} $T$ \textsf{ELSE NULL END)}\\
\textsf{\,\,\,\,\,\,\,\,AS N1,}\\
\textsf{\,\,\,\,PERCENTILE\_CONT(0.5) WITHIN GROUP (}\\
\textsf{\,\,\,\,\,\,\,\,ORDER BY CASE WHEN} $A_p=v_2$ \textsf{THEN} $T$ \textsf{ELSE NULL END)}\\
\textsf{\,\,\,\,\,\,\,\,AS median2,}\\
\textsf{\,\,\,\,COUNT(CASE WHEN} $A_p=v_2$ \textsf{THEN} $T$ \textsf{ELSE NULL END)}\\
\textsf{\,\,\,\,\,\,\,\,AS N2}\\
\textsf{FROM discretized}\\
\textsf{GROUP BY} $A_1, ..., A_n$\textsf{,}\\
\textsf{HAVING}\\
\textsf{\,\,\,\,PERCENTILE\_CONT(0.5) WITHIN GROUP (}\\
\textsf{\,\,\,\,ORDER BY CASE WHEN} $A_p=v_1$ \textsf{THEN} $T$ \textsf{END) <}\\
\textsf{\,\,\,\,PERCENTILE\_CONT(0.5) WITHIN GROUP (}\\
\textsf{\,\,\,\,ORDER BY CASE WHEN} $A_p=v_2$ \textsf{THEN} $T$ \textsf{END)}\\
\textsf{),}\\
\textsf{inter\_table AS (}\\
\textsf{SELECT} $A_1, ..., A_n, T, A_p$ \textsf{,total\_median}\\
\textsf{FROM discretized INNER JOIN filtered USING} $(A_1, ..., A_n)$ \\
\textsf{),}\\
\textsf{observed AS (}\\
\textsf{SELECT }$A_1,...,A_n$\textsf{,}\\
\textsf{\,\,\,\,COUNT(CASE WHEN} $A_p=v_1$ \textsf{AND} $T$\textsf{>total\_median THEN} $T$\\
\textsf{\,\,\,\,\,\,\,\,\,\,\,\,\,\,\,\,\,\,\,\,\,\,\,\,END) AS v1\_over,}\\                  
\textsf{\,\,\,\,COUNT(CASE WHEN} $A_p=v_2$ \textsf{AND} $T$\textsf{>total\_median THEN} $T$\\
\textsf{\,\,\,\,\,\,\,\,\,\,\,\,\,\,\,\,\,\,\,\,\,\,\,\,END) AS v2\_over,}\\
\textsf{\,\,\,\,COUNT(CASE WHEN} $A_p=v_1$ \textsf{AND} $T$\textsf{<=total\_median THEN} $T$\\
\textsf{\,\,\,\,\,\,\,\,\,\,\,\,\,\,\,\,\,\,\,\,\,\,\,\,END) AS v1\_under,}\\
\textsf{\,\,\,\,COUNT(CASE WHEN} $A_p=v_2$ \textsf{AND} $T$\textsf{<=total\_median THEN} $T$\\
\textsf{\,\,\,\,\,\,\,\,\,\,\,\,\,\,\,\,\,\,\,\,\,\,\,\,END) AS v2\_under}\\
\textsf{FROM inter\_table}\\
\textsf{GROUP BY} $A_1, ..., A_n$\textsf{)}\\
\\
\textsf{SELECT *} \\
\textsf{FROM observed NATURAL INNER JOIN filtered}\\
\textsf{WHERE v1\_over+v1\_under>=}$M$ \textsf{AND v2\_over+v2\_under>=}$M$\textsf{;}


\end{tabular}
\end{center}
\vspace{-2mm}
\end{tcolorbox}
\end{minipage}%%
\vspace{-4mm}
\caption{Median aggregation query for a given attribute combination $A_1,\ldots, A_n$ }
\label{fig:full_median_gb_query}
\end{figure}
